Semantic Shift Estimation via Dual-Projection and Classifier Reconstruction for Exemplar-Free Class-Incremental Learning

Exemplar-Free Class-Incremental Learning (EFCIL) aims to sequentially learn from distinct categories without retaining exemplars but easily suffers from catastrophic forgetting of learned knowledge. While existing EFCIL methods leverage knowledge distillation to alleviate forgetting, they still face two critical challenges: semantic shift and decision bias. Specifically, the embeddings of old tasks shift in the embedding space after learning new tasks, and the classifier becomes biased towards new tasks due to training solely with new data, hindering the balance between old and new knowledge. To address these issues, we propose the Dual-Projection Shift Estimation and Classifier Reconstruction (DPCR) approach for EFCIL. DPCR effectively estimates semantic shift through a dual-projection, which combines a learnable transformation with a row-space projection to capture both task-wise and category-wise shifts. Furthermore, to mitigate decision bias, DPCR employs ridge regression to reformulate a classifier reconstruction process. This reconstruction exploits previous in covariance and prototype of each class after calibration with estimated shift, thereby reducing decision bias. Extensive experiments demonstrate that, on various datasets, DPCR effectively balances old and new tasks, outperforming state-of-the-art EFCIL methods. Our codes are available at https://github.com/RHe502/ICML25-DPCR.

==> sec/3_preliminary.tex <==
\section{Preliminary}
\label{sec:preliminary}

\subsection{Problem Setting of EFCIL}
Prior to further description, we provide definitions of EFCIL here. In EFCIL, the model learns from training data in a task-wise manner. For an EFCIL problem consisting $T$-tasks, in task $t$, the model learns from the dataset $\mathcal{D}_{t}=\{\mathcal{X}_{t,i}, y_{t,i}\}_{i=1}^{N_{t}}$, where $\mathcal{X}_{t,i} \in \mathbb{R}^{ c\times w \times h}$ denotes the $i$-th input data with the shape of $c \times w \times h$ in task $t$, $y_{t,i}$ denotes the label of the $i$-th input data, and $N_t$ is the total number of samples in task t. The label set of task $t$ is denoted as $\mathcal{C}_t$ and $\mathcal{C}_i \cap \mathcal{C}_j = \emptyset (i \ne j)$ in EFCIL. In this paper, we focus on the cold-start setting, where the model is initialized randomly and unlike the warm-start setting and the first task in cold-start setting contains the same number of categories as other tasks (i.e., $|\mathcal{C}_{0}|$ = $|\mathcal{C}_{j}| = C, j\in1:T$). In task $t$, the backbone is denoted as $f_{\theta_{t}}: \mathbb{R}^{ c\times w \times h} \rightarrow \mathbb{R}^{d}$ (parameterized by $\theta_t$) and the embeddings extracted by the backbone is classified via a mapping 
% $h_{\tau_{t}}: \mathbb{R}^{d} \rightarrow \mathbb{R}^{l_{t}}$ (parameterized by $\tau_t$),
$\mathbb{R}^{d} \rightarrow \mathbb{R}^{l_{t}}$,
where $d$ is the feature dimension and $l_t = tC$ is the number of classes that the model have met. The goal of EFCIL is to train the model with $\mathcal{D}_{t}^{\text{train}}$ at task $t$ without access of data from previous tasks and validate the model on $\mathcal{D}_{1:t}^{\text{test}}$ after training in task $t$. 
% {\color{red} Add the definition of warm-start (cold-start) setting.}

\subsection{Ridge-regression Classifier} \label{ssec:rr}
In this paper, we leverage the ridge-regression to address the bias in classifier training. Here, we provide the details of ridge-regression classifier training. The classifier  ${h}_{\bm{W}_{t}}$ is a full-connected layer parameterized by $\bm{W}_{t}$. In task $t$, suppose the $i$-th input data's embeddding  extracted by the backbone $\theta_{t}$ is denoted as $x_{t,i}^{\theta_{t}} = f_{\theta_{t}}(\mathcal{X}_{t,i})$ and the onehot label is $\onehot{y_{t,i}}$, the embeddings and one-hot label of all the input data can be stacked as $\bm{X}_{t}^{\theta_{t}}$ and $\bm{Y}_{t}$ respectively, where
\begin{equation}\label{eq_emb_label}
	\resizebox{0.42\textwidth}{!}{$\bm{X}_{t}^{\theta_t} = \begin{bmatrix}
		\bm{x}_{t,1}^{\theta_{t}} \\
		\bm{x}_{t,2}^{\theta_{t}} \\
		\vdots \\
		\bm{x}_{t,N_1}^{\theta_{t}}
	\end{bmatrix} = \begin{bmatrix}
		f_{\theta_{t}}(\mathcal{X}_{t,1}) \\
		f_{\theta_{t}}(\mathcal{X}_{t,2}) \\
		\vdots \\
		f_{\theta_{t}}(\mathcal{X}_{t,N_1})
	\end{bmatrix} \quad
	\bm{Y}_{t} = \begin{bmatrix}
		\onehot{y_{t,1}} \\
		\onehot{y_{t,2}} \\
		\vdots       \\
		\onehot{y_{t,N_1}}
	\end{bmatrix}$}.
\end{equation}

If given the joint learning problems from task 1 to $t$ with dataset $\mathcal{D}_{1:t}^{\text{train}} = \mathcal{D}_{1}^{\text{train}} \cup \mathcal{D}_{2}^{\text{train}} \cup ... \cup \mathcal{D}_{t}^{\text{train}}$, the embeddings after the corresponding backbone $\theta_i,i\in1:t$ and the labels can be stacked to form $\bm{X}_{1:t}^{\theta_1}$ and $\bm{Y}_{1:t}$.
\begin{equation}\label{eq_stack_task}
	\bm{X}_{1:t}^{\theta_1} = \begin{bmatrix}
		\bm{X}_{1}^{\theta_1} \\
		\bm{X}_{2}^{\theta_1} \\
		\vdots \\
		\bm{X}_{t}^{\theta_1}
	\end{bmatrix}
	 \quad
	\bm{Y}_{1:t} = \begin{bmatrix}
		\bm{Y}_{1} \\
		\bm{Y}_{2} \\
		\vdots       \\
		\bm{Y}_{t}
	\end{bmatrix}.
\end{equation}
Then the joint learning problem can be formulated as follows 
\begin{align}\label{eq_L2_all}
	\argmin{\bm{W}_{t}} \quad \lVert\bm{Y}_{1:t} - \bm{X}_{1:t}^{\theta_1}\bm{W}_{t}\rVert_{\text{F}}^{2} + {\gamma} \left\lVert\bm{W}_{t}\right\rVert_{\text{F}}^{2}, 
\end{align}
where $\lVert\cdot\rVert_{\text{F}}$ is Frobenius-norm, $\gamma$ is the regularization factor of ridge-regression and $\bm{W}_{\text{t}}$ is the optimal weight for all the tasks that have seen. The optimal solution to Eq. \eqref{eq_L2_all} is 
\begin{align}
	\nonumber \bm{\hat W}_{t} & = (\bm{X}_{1:t}^{\theta_{t}\T}\bm{X}_{1:t}^{\theta_{t}}+\gamma \bm{I})^{-1}\bm{X}_{1:t}^{\theta_{t}\T}\bm{Y}_{1:t} \\ \label{eq_ls_w_all}
    &= (\sum_{i=1}^{t}\bm{X}_{i}^{\theta_{t}\T}\bm{X}_{i}^{\theta_{t}}+\gamma \bm{I})^{-1}\sum_{i=1}^{t}\bm{X}_{i}^{\theta_{t}\T}\bm{Y}_{i},
\end{align}
where ${\cdot}^ {\T}$ denotes transpose operation and $\bm{I}$ is the identity matrix. Here we denote the uncentered covariance of task $i$ $\bm{X}_{i}^{\theta_{t}\T}\bm{X}_{i}^{\theta_{t}}$ as $\Phi_{i}^{\theta_1}$ and the correlation $\bm{X}_{i}^{\theta_{t}\T}\bm{Y}_{i}$ as $\bm{H}_{i}^{\theta_1}$, the Eq. \eqref{eq_ls_w_all}
can be rewritten as
\begin{align} \label{eq_ls_rq}
	\bm{\hat W}_{t}  = (\sum_{i=1}^{t}\Phi_{i}^{\theta_1}+\gamma \bm{I})^{-1}\sum_{i=1}^{t}\bm{H}_{i}^{\theta_1}.
\end{align}

As shown in Eq. \eqref{eq_ls_rq}, the classifier can be constructed covariance and correlation of data in each tasks without directly accessing previous data or embeddings. That is, the previous information can be encoded in $\Phi_{i}^{\theta_t}$ and $\bm{H}_{i}^{\theta_t}$ and the new information $\Phi_{t}^{\theta_t}$ and $\bm{H}_{t}^{\theta_t}$ can be calculated directly and the classifier can be reconstructed. The reconstruction comes from the joint optimization and the classifier is not updated from previous tasks then avoid the balance issue. However, due to the constrain of EFCIL, the embeddings 

\textbf{Category-wise Implementation of RR.} From the viewpoint of each category, we can delve deeper into the covariance and correlation matrices and construct classifiers in a category-specific manner. For $\bm{\Phi}_{i}^{\theta_{i}}$ and $\bm{H}_{i}^{\theta_{i}}$ obtained after task $i$ with the backbone $\theta_i$, they can be rewritten as
\begin{align} \nonumber 
    \bm{\Phi}_{i}^{\theta_{i}} &= \bm{X}_{i}^{\theta_{t-1}\T}\bm{X}_{i}^{\theta_{i}} =\sum_{c \in \mathcal{C}_{i}}^{|\mathcal{C}_{i}|}\bm{X}_{i,c}^{\theta_{i}\T}\bm{X}_{i,c}^{\theta_{i}} =\sum_{c \in \mathcal{C}_{i}}^{|\mathcal{C}_{i}|}\bm{\Phi}_{i,c}^{\theta_{i}}, \\ \label{eq_rq_class}
    \bm{H}_{i}^{\theta_{i}} &= \bm{X}_{i}^{\theta_{i}\T}\bm{Y}_{i} =\sum_{c \in \mathcal{C}_{i}}^{|\mathcal{C}_{i}|}\bm{X}_{i,c}^{\theta_{i}\T}\bm{Y}_{i,c} =\sum_{c \in \mathcal{C}_{i}}^{|\mathcal{C}_{i}|}\bm{H}_{i,c}^{\theta_{i}},
\end{align}
where $\bm{X}_{i,c}^{\theta_{i}}$ is the embedding matrix of class $c$ in task $i$ and  $\bm{Y}_{i,c}$ contains the the one-hot label of class $c$ in task $i$. 

Via the decomposition in Eq. \eqref{eq_rq_class}, we can further encode the $\bm{H}_{i}^{\theta_{i}}$ with the prototype (i.e., mean of embeddings) of each class in task $i$, that is 
\begin{align} \label{eq_proto}
    \bm{H}_{i}^{\theta_{i}} = \sum_{c \in \mathcal{C}_{i}}^{C} N_c \bm{\mu}_{i,c}^{\theta_{i}\T}\bm{y}_{i,c},\quad
    \bm{\mu}_{i,c}^{\theta_{i}} = \frac{1}{N_c} \sum_{j=1}^{N_c} \bm{x}_{i,c,j}^{\theta_{i}}, 
\end{align}
where $N_c$ is the number of samples of class $c$. With Eq. \eqref{eq_proto}, we can store the prototype of each class then reform the correlation matrix with labels. This operation can reduce the memory footprint of $d \times tC$ to $d$ for each class. 

\subsection{Framework of Existing ACL Methods} \label{ssec:acl}
% ACL solves the incremental problem in a linear classifier attached behind a feature extractor via recursive operations. 

\textbf{Conditional Weight-invariance in ACL.} From Eq. \eqref{eq_ls_rq}, with the frozen backbone, ACL can use the information of all tasks to construct the classifier without directly accessing previous data or embeddings. That is, the previous information can be encoded in $\Phi_{i}^{\theta_1}$ and $\bm{H}_{i}^{\theta_1}$ and the new information $\Phi_{t}^{\theta_1}$ and $\bm{H}_{t}^{\theta_1}$ can be calculated directly. Since the solution in Eq. \eqref{eq_ls_rq} is based on the joint learning problem of Eq. \eqref{eq_L2_all}, implementing Eq. \eqref{eq_ls_rq} by adding up $\Phi_{i}^{\theta_1}$ and $\bm{H}_{i}^{\theta_1}$ in task $t$ will be identical to results of joint learning if $\Phi_{i}^{\theta_1}$ and $\bm{H}_{i}^{\theta_1}$ are stored and stay unchanged (i.e. freeze the backbone). This brings the weight-invariant property of ACL in the classifier \cite{ACIL2022NeurIPS}. 

\textbf{Dilemma in existing ACL framework.} However, the weight-invariance is based on the same frozen backbone $\theta_1$ (see Eq. \eqref{eq_ls_w_all}) and this may cause less effective representation of unseen categories \cite{REAL2024}. Freezing backbone maybe fine in the warm-start setting, but in the cold-start setting, the decision boundary built upon  $\theta_1$ may not capable of separating new classes. If backbone is updated to new tasks, semantic shift of embeddings happens and can $\Phi_{i}^{\theta_1}$ and $\bm{H}_{i}^{\theta_1}$ become sub-optimal. Then decision boundary constructed by them will be misaligned with shifted embeddings. This causes the dilemma of representation adaption in ACL. To overcome this problem, we should both adapt the backbone to new tasks while keep decision boundaries aligned with the representation. In this paper, we propose DPR to achieve this goal.
It is worth mentioned that, we provide a different implementation form of ACL to give a better insight, and this implementation is equivalent to that proposed in the original ACL framework \cite{ACIL2022NeurIPS}. Please refer to Appendix \ref{sec:acl} to check the equivalence between two implementations. 


% Also, this category-wise implementation facilitates the derivation of our DPR (see Section \ref{sec:method}).

% \begin{itemize}
%     \item {\color{red} Backbone training in first tasks.}
%     \item {\color{red} Formulation of ridge-regression classification.}
%     \item {\color{red} Extend the first task to following tasks.}
%     \item {\color{red} The drawback of existing ACL.}
% \end{itemize}

